How to Make an Image More Memorable? A Deep Style Transfer Approach

Recent works have shown that it is possible to automatically predict intrinsic image properties like memorability. In this paper, we take a step forward addressing the question: "Can we make an image more memorable?". Methods for automatically increasing image memorability would have an impact in many application fields like education, gaming or advertising. Our work is inspired by the popular editing-by-applying-filters paradigm adopted in photo editing applications, like Instagram and Prisma. In this context, the problem of increasing image memorability maps to that of retrieving "memorabilizing" filters or style "seeds". Still, users generally have to go through most of the available filters before finding the desired solution, thus turning the editing process into a resource and time consuming task. In this work, we show that it is possible to automatically retrieve the best style seeds for a given image, thus remarkably reducing the number of human attempts needed to find a good match. Our approach leverages from recent advances in the field of image synthesis and adopts a deep architecture for generating a memorable picture from a given input image and a style seed. Importantly, to automatically select the best style a novel learning-based solution, also relying on deep models, is proposed. Our experimental evaluation, conducted on publicly available benchmarks, demonstrates the effectiveness of the proposed approach for generating memorable images through automatic style seed selection

==> conclusions.tex <==


%Discussion

To the best of our knowledge we are the First work showing that show it is possible to automatically increase memorability using a style transfer approach.
For this reason, a direct comparison with previous related work is not possible.
Indeed, even recent work Khosla show that it is possible to reproduce a faithful memorability map, which can be used as a base for further image manupulations. Still, their method do not produce memorability increase.
The only work on increasing memorability is on faces and cannot be directly applied in our settings, with generic images.

While literature on predicting image abstract concepts like memorability is quite huge, the literature in image synthesis is still in its early infancies.

Other approaches for image synthesis based on style transfer can be embedded in our method. We use the one from Ulyanov rather than Gatys and [...] but Ulyanov's stylization process is the fastest to generate our training samples for training the Selector. 

We plan to investigate Argument why we did not use GANs(?)
The choice of architecture is to keep the user in the loop and allow him/her a range of creativity/freedom on the style selection.
%Future work for ACM MM: 

% Conclusion
We also provide a lightweight solution which can efficiently learn from a limited set of matches, allowing the seed retrieval from a relatively large set of candidate seeds, thus increasing the potential user creativity space, while dramatically reducing the number of training matches required.
Focusing on memorability transfer based on low level cues, %thus discarding the effect of semantic, 
we use abstract art paintings from the DeviantArt dataset as our seed images. 


the advantages:
1) partial training set
2) provide a ranking at test time
3) avoid running style transfer at test time.

limitation:
1) we cannot add a new seed without a long retraining process


Our method is generic and potentially may be applied for other concepts like aesthetic judgement or emotions. 
Methods for automatically increasing image memorability would have an impact in many application fields like education, gaming or advertising.
For example, students would like to remember interesting things with less effort and companies would like to increase the chances of their logo or ads to be remembered.  

Also, in a photo editing application scenario, the ideal situation would be that a user may be able to fine tune for example the desired level of memorability rather than aesthetic.
A multi-concepts style seed selector may be an interesting use case study for the future.

Another interesting extension of the method may be to perform an analysis based the image category such as portrait, landscape, streetscape, etc. For example, the method may automatically discover the best styles for different categories.




All these findings motivate us to pursue this line of research and to develop a methodological framework that is able to automatically increase the memorability of an input set of images. Our understanding is that the method should be able to do that (i) in an efficient manner, (ii) without significant modifications of the high-level image content and (iii) at the same time as selecting the subset of images that is going to have the highest memorability once they are modified. Such tool may have direct impact in fields like education, elderly care or user-generated data analysis. Indeed, rapidly selecting the most memorable images among all possible high-level content preserving modifications of the initial image set could help editing better educational supports, designing more effective brain training games for elderly people or producing better summaries from lifelog camera image streams or leisure picture albums.
